SCOPE: Score-Isolated Agentic Optimization for Video World Models

Video world models are increasingly used as simulators for planning and embodied decision making, yet improving them at inference time introduces a subtle evaluation problem: prompts, samplers, verifiers, and selectors may evolve together, making it difficult to attribute gains or prevent held-out feedback from shaping the final policy. We introduce \scope (\emph{\scopefullname}), a framework for auditable inference-time adaptation of frozen video world models. \scope represents external controls as a typed state, updates this state only through bounded changes supported by development evidence, and freezes the resulting policy before held-out evaluation. On Physics-IQ benchmark, \scope improves over the exact frozen base by $+14.24$ (95\% CI $[+8.10,+21.23]$). Controlled ablations further identify gains from scene specification, sampling, and learned selection, while the margin over the strongest matched agentic baseline remains unresolved. Cross-backbone and prospective evaluations reveal a complementary result: useful inference-time updates exist, but their benefits do not transfer uniformly across models and settings. Together, these findings suggest that reliable inference-time adaptation requires not only better proposals, but also a principled mechanism for deciding which updates should become part of the deployed system. Code is available at https://github.com/YuhuaJiang2002/SCOPE.

==> core_claim_ablation_rows.tex <==
\multicolumn{4}{@{}l}{\emph{A. Control dimensions (protocol-local; not additive)}}\\
\textbf{Text control} & SceneLang vs exact Base (66 scenes; seeds 0--2) & $+5.62\;[+0.55,+10.55]$ P-IQ & credited component\\
\textbf{Noise control} & CFG/step edit vs matched SceneLang (66 scenes; 4 seeds) & $+1.26\;[+0.52,+2.01]$ P-IQ & credited; guards pass\\
\textbf{Reward control} & supervised Bo16 vs random / self-score (64 scenes) & $+3.33\;[+1.49,+5.30]$ / $+0.66\;[-1.52,+2.92]$ P-IQ & credited only vs random\\
\midrule
\multicolumn{4}{@{}l}{\emph{B. Skill optimization and governance ablations}}\\
\textbf{No evolution ($\Omega_0$)} & frozen incumbent skill (40 scenes) & $24.16$ absolute P-IQ & reference skill\\
\textbf{Random update} & matched update budget vs $\Omega_0$ (40 scenes) & $28.70$; $+4.53\;[+1.14,+9.17]$ vs $\Omega_0$ & positive control\\
\textbf{Typed update ($\Omega_1$)} & typed transfer vs $\Omega_0$; then matched random (40 scenes) & $28.38$; $+4.22\;[+0.81,+8.30]$ vs $\Omega_0$; $-0.32\;[-5.98,+5.15]$ vs random & blocked; harm $15\%$\\
\textbf{Remove fallback} & retirement vs commit+fallback (32 tasks) & $-0.773\;[-1.471,-0.203]$ Overall & fallback is necessary\\
\midrule
\multicolumn{4}{@{}l}{\emph{C. Complete method on the 40-scene common-base Physics-IQ protocol}}\\
\textbf{Full \scope{} (ours)} & exact Base $20.70$; strongest Qwen $32.87$ (same 40 scenes) & \textbf{$34.94$ (rank 1); $+14.24\;[+8.10,+21.23]$ vs Base}; $+2.07\;[-0.27,+6.14]$ vs Qwen & \textbf{best point estimate; Base gain confirmed}\\


==> opens2v_crossbackbone_rows.tex <==
% Generated by publish_crossbackbone_panels.py
% source_rows_sha256=25547b77dbf455806fb13203364a7419e44e11a6447717ad4faf810b4154acfb
Frozen Base~\citep{wan2025,yang2025cogvideox} & $37.46$ & $36.60$ & $48.30$ & $48.29$\\
Qwen-Image-Agent-style~\citep{qwenimageagent2026} & $38.72$ & $37.92$ & $46.73$ & $46.16$\\
LingBot-style Director$\to$Pilot prompt proxy$^\ddagger$~\citep{lingbotworld2026} & $41.27$ & $42.84$ & $47.39$ & $\mathbf{49.62}$\\
GPT-5.4 first-frame skill (internal) & $38.31$ & $39.33$ & $46.67$ & $47.99$\\
\scope{} (ours) & $\mathbf{41.75}$ & $\mathbf{43.17}$ & $\mathbf{47.76}$ & $49.22$\\


==> pai_crossbackbone_rows.tex <==
% Generated by publish_crossbackbone_panels.py
% source_rows_sha256=66405aa24484d766e1adfebd10571c4aa886efa47e8faaf0ebc384691e572301
\multicolumn{5}{@{}l}{\emph{Ranking-eligible matched methods}}\\
Frozen Base & $76.67$ & -- & $74.10$ & --\\
$+$ shared global & $76.86$ & $+0.19$ {\scriptsize CI $[-2.13,+2.66]$} & $74.41$ & $+0.30$ {\scriptsize CI $[-2.15,+2.77]$}\\
LingBot-style Director$\to$Pilot $+$ shared global$^\dagger$ & $76.77$ & $+0.10$ {\scriptsize CI $[-2.25,+2.54]$} & $74.29$ & $+0.18$ {\scriptsize CI $[-2.30,+2.69]$}\\
Qwen-Image-Agent-style (SceneLang) & $77.02$ & $+0.35$ {\scriptsize CI $[-1.50,+2.32]$} & $\mathbf{74.72}$ & $\mathbf{+0.62}$ {\scriptsize CI $[-1.37,+2.68]$}\\
SceneLang $+$ shared global & $77.01$ & $+0.34$ {\scriptsize CI $[-1.86,+2.63]$} & $71.57$ & $-2.53$ {\scriptsize CI $[-5.25,+0.12]$}\\
\midrule
\multicolumn{5}{@{}l}{\emph{Post-hoc upper envelope; no ranking or promotion credit}}\\
\scope{} post-hoc upper envelope$^{*}$ & $\mathbf{77.47}$ & $\mathbf{+0.80}$ {\scriptsize CI $[-1.38,+3.12]$} & $74.48$ & $+0.38$ {\scriptsize CI $[-1.56,+2.37]$}\\


==> pai_full_metrics_unified72_eight_dimension_rows.tex <==
Frozen base (absolute) & 89.51 & 91.71 & 98.49 & 44.21 & 62.83 & 19.50 & 92.44 & 95.75 \\
Shared global (Base parent) & -0.45 & -0.18 & -0.73 & +0.61 & +1.60 & -0.12 & -0.09 & -0.02 \\
Qwen-Image-Agent-style (SceneLang)~\citep{qwenimageagent2026} & +0.89 & +0.37 & +0.13 & +0.42 & +0.50 & -0.06 & +0.66 & +0.49 \\
SceneLang + shared global & -0.03 & +0.19 & -0.65 & +0.79 & +2.25 & -0.04 & +0.10 & +0.03 \\
LingBot-style + safe fallback$^\dagger$~\citep{lingbotworld2026} & +0.24 & +0.10 & +0.03 & 0.00 & +0.28 & -0.02 & +0.13 & +0.12 \\
LingBot-style Director$\to$Pilot + shared global$^\dagger$~\citep{lingbotworld2026} & -0.16 & +0.02 & -0.70 & +0.70 & +2.17 & -0.22 & +0.06 & +0.07 \\
LingBot-style Director$\to$Pilot (raw)~\citep{lingbotworld2026} & +1.33 & +0.49 & +0.26 & -0.24 & +0.94 & +0.12 & +0.58 & +0.64 \\
LingBot-style + shared global & +0.15 & +0.22 & -0.55 & +0.60 & +1.73 & -0.26 & -0.08 & +0.15 \\
GPT-5.4-SKILL (raw) & -1.02 & -1.61 & +0.07 & -1.41 & -0.09 & +0.09 & +0.14 & +0.72 \\
GPT-5.4-SKILL + shared global & -2.67 & -2.27 & -0.66 & -1.64 & -1.14 & -0.24 & -0.54 & +0.07 \\
\midrule
\scope{} w/o shared global$^\ddagger$ & +0.81 & +0.36 & +0.13 & +0.41 & +0.57 & -0.01 & +0.61 & +0.44 \\
\textbf{\scope{} + shared global (ours)$^\ddagger$} & -0.06 & +0.20 & -0.68 & +0.69 & +2.33 & -0.03 & 0.00 & +0.02 \\


==> physiq_common_base_crossbackbone_rows.tex <==
% Generated by publish_scope_cogvideox_common_base_panel.py --phase tex
% panel_result_sha256=3d9605eb30e97091dd61359d5ad31fb79a32cea3e44339c181c211a8fa91845b
% lingbot_result_sha256=d68ef53bcefb9fcf4ae7045bd4ed560d2576d841014cc81834169383e3de1d4a
Frozen Base & $20.70$ & -- & $22.91$ & --\\
WMReward reward-only~\citep{wmreward2026} & $21.81$ & $+1.11\;[-0.40,+3.17]$ & $26.10$ & \meas{$+3.19\;[+0.85,+6.04]$}\\
VAE-$\theta$ reward & $22.33$ & $+1.63\;[-0.67,+4.46]$ & $25.14$ & \meas{$+2.23\;[+0.02,+4.83]$}\\
VIGOR reward-only~\citep{vigor2026} & $25.15$ & \meas{$+4.44\;[+1.49,+7.96]$} & $27.75$ & \meas{$+4.83\;[+1.71,+8.44]$}\\
uniform random 3-candidate selector~\citep{brown2024large,ma2025inference} & $27.41$ & \meas{$+6.71\;[+1.93,+11.45]$} & $30.57$ & \meas{$+7.65\;[+4.51,+10.97]$}\\
LingBot-style Director$\to$Pilot proxy$^\dagger$~\citep{lingbotworld2026} & $29.98$ & \meas{$+9.27\;[+2.37,+16.12]$} & $34.91$ & \meas{$+12.00\;[+6.76,+17.62]$}\\
fixed GPT-5.4 physics card & $30.04$ & \meas{$+9.33\;[+2.50,+15.93]$} & $34.89$ & \meas{$+11.98\;[+7.05,+17.13]$}\\
fixed rule refinement & $31.50$ & \meas{$+10.80\;[+2.67,+19.14]$} & $33.89$ & \meas{$+10.98\;[+6.27,+15.93]$}\\
joint self-score ablation & $32.07$ & \meas{$+11.37\;[+3.38,+19.69]$} & $34.63$ & \meas{$+11.71\;[+6.83,+16.66]$}\\
Qwen-Image-Agent-style feedback~\citep{qwenimageagent2026} & $32.87$ & \meas{$+12.16\;[+4.48,+20.06]$} & $34.99$ & \meas{$+12.08\;[+7.36,+16.98]$}\\
\textbf{\textsc{SCOPE} (ours)} & \meas{$\mathbf{34.94}$} & \meas{$\mathbf{+14.24\;[+8.10,+21.23]}$} & \meas{$\mathbf{35.51}$} & \meas{$\mathbf{+12.60\;[+7.73,+17.60]}$}\\


==> physiq_s115_lingbot_claims_generated.tex <==
% Generated by publish_physiq_s115_lingbot_paper_claims.py; do not edit.

% status: matched_11_method_scene_mean_table1_claims

\newcommand{\ScopeCommonBaseAbstractClaim}{%
On the matched 40-scene Physics-IQ benchmark, \scope achieves $34.94$ and improves
over Base by $+14.24$ (95\% CI $[+8.10,+21.23]$). Its $+2.07$ advantage over the
strongest matched non-\scope baseline remains unresolved
(CI $[-0.27,+6.14]$). A descriptive same-candidate analysis further shows a
$+7.53$ gain over uniform selection (CI $[+4.04,+11.52]$).
}

\newcommand{\ScopeCommonBaseCoreContribution}{%
Under the matched 40-scene Physics-IQ protocol, \scope achieves the highest point
estimate ($34.94$) and outperforms uniform selection over the same three generated
candidates by $+7.53$ (CI $[+4.04,+11.52]$;
Section~\ref{sec:physiq-common-base}).
}

\newcommand{\ScopeCommonBaseBoundaryContribution}{%
The strongest matched non-\scope comparator, Qwen-Image-Agent-style feedback,
scores $32.87$; the resulting $+2.07$ margin for \scope remains unresolved
(CI $[-0.27,+6.14]$). Prospective evaluations further show that these
within-protocol gains do not establish generalization to unseen tasks
(Section~\ref{sec:integrated}).
}

\newcommand{\ScopeCommonBaseResultParagraph}{%
Table~\ref{tab:headline} compares eleven methods under a matched evaluation
protocol: all methods share the same 40 scenes, official scorer, candidate pool,
and Base reference within each backbone. The retrospective LingBot
Director$\to$Pilot baseline follows the same generation and evaluation protocol.
Following a post-score materialization failure, its score evidence was recovered
by deterministic replay of the original hash-bound videos, without additional
selection or tuning.

On Wan2.2, \scope achieves the highest point estimate at $34.94$, compared with
$32.87$ for the strongest non-\scope method, Qwen-Image-Agent-style feedback.
The resulting $+2.07$ difference remains unresolved
(CI $[-0.27,+6.14]$). LingBot obtains $29.98$, corresponding to a $+9.27$
improvement over Base (CI $[+2.37,+16.12]$). Its nonlinear full-set aggregate
($23.57$) is reported separately and is not included in the scene-mean ranking.

The clearest matched result is the comparison with Base: \scope improves
Physics-IQ by $+14.24$ (CI $[+8.10,+21.23]$). A descriptive analysis that holds
the three generated candidates fixed also yields a $+7.53$ improvement over
uniform selection (CI $[+4.04,+11.52]$). This latter comparison controls for
candidate generation, but was not designated as the primary contrast.
}

\newcommand{\ScopeCommonBaseTableCaptionClaim}{%
All rows report the mean over 40 scene-level Physics-IQ composites. Within each
backbone, methods share the same Base and evaluation protocol. The \scope--Qwen
differences are $+2.07$ on Wan (CI $[-0.27,+6.14]$) and $+0.52$ on CogVideoX
(CI $[-0.39,+1.65]$), and remain unresolved on both backbones. Absolute scores
are not compared across backbones. The dagger denotes the separately generated
fixed Director baseline; \meas{green} indicates Base-relative intervals with
positive lower bounds.
}

\newcommand{\ScopeLingBotTableExtension}{}

\newcommand{\ScopeCommonBaseAblationCaptionClaim}{%
The final row reports the complete \scope method. On the matched 40-scene
Physics-IQ protocol, \scope achieves the highest point estimate ($34.94$) and
improves significantly over exact Base. Its $+2.07$ difference from Qwen remains
unresolved (CI $[-0.27,+6.14]$).
}

\newcommand{\ScopeCommonBaseAblationRankClaim}{%
absolute rankings are therefore interpreted only within the matched common-base
Physics-IQ protocol.
}

\newcommand{\ScopeCommonBaseDiscussionClaim}{%
On the matched 40-scene Physics-IQ protocol, \scope improves over exact Base by
$+14.24$ (CI $[+8.10,+21.23]$) and achieves the highest point estimate at $34.94$.
The strongest non-\scope method, Qwen-Image-Agent-style feedback, scores $32.87$;
their $+2.07$ difference remains unresolved (CI $[-0.27,+6.14]$).
A descriptive same-candidate comparison additionally shows a $+7.53$ gain over
uniform selection (CI $[+4.04,+11.52]$). These results establish improvement
within this matched protocol, but do not by themselves imply unseen-task
generalization.
}

\newcommand{\ScopeCommonBaseConclusionClaim}{%
the matched \scope policy improves over uniform selection of the same three
candidates by $+7.53$ in a descriptive analysis, while its $+2.07$ advantage
over Qwen-Image-Agent-style feedback remains unresolved
(CI $[-0.27,+6.14]$).
}

\newcommand{\ScopeMatchedLingBotReproducibility}{%
The retrospective LingBot comparison is reproduced under the same matched
Physics-IQ protocol and linked to its generation, scoring, and replay records in
the release manifest. Its Table~1 results and dependent claims are regenerated
by the corresponding baseline and paper-claim scripts.
}

==> scope_common_base_first_four_rounds_generated.tex <==

% Generated by plot_scope_first_four_rounds.py
% wan_result_sha256=9267a360f5a7658ce9ca83619213a243991691e2c1ac92c6d523783d0b923860
% cogvideox_result_sha256=aa4fbd6bbb02afb13ca13b054c1019edb202a0b6a6129fb3d95bd82079089886

\newcommand{\ScopeActualEvolutionTableRows}{%
%
}

\newcommand{\ScopeEvolutionCaption}{%
\textbf{Evolution of the matched Physics-IQ policy across two frozen backbones.}
R0--R3 correspond to Base, the physics-card update, the rule-refinement update,
and the final selected \scope state. Curves show the mean Physics-IQ score over
40 scenes, with shaded 95\% scene-bootstrap confidence intervals.
Scores are compared only within each backbone.%
}

\newcommand{\ScopeEvolutionParagraph}{%
Figure~\ref{fig:scope-common-base-evolution} shows how the matched policy evolves
through the four states used to construct the final \scope policy. On Wan2.2,
Physics-IQ increases from $20.70$ at Base to $30.04$, $31.50$, and $34.94$
across R1--R3. On CogVideoX, the corresponding trajectory is
$22.91\to34.89\to33.89\to35.51$. Despite the intermediate decrease at R2 on
CogVideoX, the final state improves substantially over the exact Base on both
backbones. This figure illustrates the evolution relative to Base rather than a
comparison with the strongest matched alternative. Additional Wan candidates
evaluated in R4--R11 did not replace the R3 state and are omitted for clarity.%
}


==> scope_prospective_tests_rows.tex <==
Fresh Physics-IQ transfer ($32$ tasks) & full \scope{} vs Base / frozen router & $+0.096\;[-0.887,+1.077]$ / $-1.019\;[-2.159,+0.146]$ & Not confirmed; gain, harm, and guard gates fail\\
Typed-update confirmation ($40$ scenes) & typed update vs matched random & $-0.316\;[-5.984,+5.145]$; harm $15\%>10\%$ & Keep incumbent; harm ceiling fails\\
Selective grounded tool router ($192{+}96$ tasks) & fit-group vs no-tool / always-on / random & $+0.083\;[-0.191,+0.381]$ / $+0.660\;[+0.016,+1.315]$ / $+0.002\;[-0.281,+0.299]$; target $+0.243$, confirm $-0.237$ & STOP; only always-on contrast resolves\\
PhyGround applicability gate ($32$ tasks) & proposal support: raw / threshold / nonnegative & $4/32$ / $0/32$ / $0/32$ (min. $8/8/4$); laws $8$ & Pre-score STOP; target and confirmation unread\\

